Improved Hardness-of-Approximation for Token Swapping

We study the token swapping problem, in which we are given a graph with an initial assignment of one distinct token to each vertex, and a final desired assignment (again with one token per vertex). The goal is to find the minimum length sequence of swaps of adjacent tokens required to get from the initial to final assignment. The token swapping problem is known to be NP-complete. It is also known to have a polynomial-time 4-approximation algorithm. From the hardness-of-approximation side, it is known to be NP-hard to approximate with ratio better than 1001/1000. Our main result is an improvement of the approximation ratio of the lower bound: We show that it is NP-hard to approximate with ratio better than 14/13. We then turn our attention to the 0/1-weighted version, in which every token has a weight of either 0 or 1, and the cost of a swap is the sum of the weights of the two participating tokens. Unlike standard token swapping, no constant-factor approximation is known for this version, and we provide an explanation. We prove that 0/1-weighted token swapping is NP-hard to approximate with ratio better than $(1-\varepsilon) \ln(n)$ for any constant $\epsilon>0$. Lastly, we prove two barrier results for the standard (unweighted) token swapping problem. We show that one cannot beat the current best known approximation ratio of 4 using a large class of algorithms which includes all known algorithms, nor can one beat it using a common analysis framework.

==> defs.tex <==
\section{Definitions and notation}

A \textsc{Token-Swapping} instance $K = (G, T, f_1, f_2)$ consists of a graph $G = (V,E)$, a set of tokens $T$ where $|T| = |V|$, and two one-to-one assignments $f_1, f_2 : T \rightarrow V$. We call $f_1$ and $f_2$ the \emph{starting} and \emph{target} configurations respectively. A swap along an edge $(u,v) \in E$ switches the locations of the tokens on $u$ and $v$. The token-swapping problem asks how many swaps are needed to arrive at the target configuration from the starting configuration. For a token-swapping instance $K$, we denote by $OPT(K)$ the length of the shortest swap sequence.

When a token $t$ lies on the vertex $v_1$ of the path $p = v_1, v_2, ..., v_k$, we use the phrase \emph{bubbling t across p} to denote the sequence of swaps $(v_1, v_2), (v_2, v_3), ..., (v_{k-1}, v_k)$.
